Pricing Public Goods for Private Sale

We consider the pricing problem faced by a seller who assigns a price to a good that confers its benefits not only to its buyers, but also to other individuals around them. For example, a snow-blower is potentially useful not only to the household that buys it, but also to others on the same street. Given that the seller is constrained to selling such a (locally) public good via individual private sales, how should he set his prices given the distribution of values held by the agents? We study this problem as a two-stage game. In the first stage, the seller chooses and announces a price for the product. In the second stage, the agents (each having a private value for the good) decide simultaneously whether or not they will buy the product. In the resulting game, which can exhibit a multiplicity of equilibria, agents must strategize about whether they will themselves purchase the good to receive its benefits. In the case of a fully public good (where all agents benefit whenever any agent purchases), we describe a pricing mechanism that is approximately revenue-optimal (up to a constant factor) when values are drawn from a regular distribution. We then study settings in which the good is only "locally" public: agents are arranged in a network and share benefits only with their neighbors. We describe a pricing method that approximately maximizes revenue, in the worst case over equilibria of agent behavior, for any $d$-regular network. Finally, we show that approximately optimal prices can be found for general networks in the special case that private values are drawn from a uniform distribution. We also discuss some barriers to extending these results to general networks and regular distributions.

==> local-open.tex <==
%\section{Discriminatory pricing}
%\label{sec:simult-D}
%
%\mfcomment{The following is taken from our board summary, July 13, 2012:}
%\begin{itemize}
%\item Mechanism should always set pricing such that an independent set is
%offered
%      the Myerson reserve price, rest get reserve price infinity.
%\item Optimal mechanism: choose the maximal independent set.
%\item We believe: NP-hard to find a vector of prices for which worst-case
%revenue
%      approximates the optimal worst-case revenue, to within $O(n^{1/2 -
%\epsilon})$.
%      --> reduction from max independent set?
%\item Nice to have: go beyond $v \sim U[0,1]$.
%\end{itemize}


\section{Sequential pricing}
\label{sec:sequential}

\subsection{Non-discriminatory pricing}
\label{sec:sequent-ND}

\mfcomment{The following is taken from our board summary, July 13, 2012:}

\begin{itemize}
    \item Assume order in which agents are offered prices is fixed in advance
and public.
    \item Each buyer considers purchasing iff neither he nor any of his
neighbors will be
      offered to again in the future.
        then buy iff value > price.
       (analysis follows that of simultaneous case).
    \item Cor1: So optimal price is always Myerson reserve price.
    \item Cor2: Revenue of best-case ordering == revenue of best-case
equilibrium in simultaneous

    \item What about worst-case ordering and worst-case revenue?
    \item Claim: there are graphs in which worst-case revenue in simultaneous is
a linear
      factor lower than the revenue for the worst-case ordering in sequential.
       Example: 5-cycle, then for each choice of 3 nodes, many nodes connected
to those 3.
       Note: difference is coming from the ability to be ``fractional" in the
simultaneous case (Difference between fractional and integral choice of whether
to purchase).
\end{itemize}

\subsection{Discriminatory pricing}
\label{sec:sequent-D}

\mfcomment{The following is taken from our board summary, July 13, 2012:}

\begin{itemize}
    \item In the clique, no commitment, optimal revenue limits (as n grows) to
0.2888..
    \item In the clique, with commitment, optimal revenue limits (as n grows) to
$1/e$

    \item Question: does it help to resell to buyers multiple times?

    \item Answer: If mechanism can choose the order, it gives back some of the
power of committing
      to prices.
       - example: commit to selling to max independent set players last.
       then even without price commitment, can offer price = infinity to those
not in
         the max independent set.
\end{itemize}

\mfcomment{The following is taken from an email sent by Brendan on July 11,
2012.}

The problem:
General graph, sell to players sequentially (possibly more than once each),
order in which the players arrive is known in advance, mechanism wants to
maximize revenue, $\epsilon = 0$, mechanism can commit to its vector of prices
in advance.

Thought: if we want to compare with the non-sequential mechanism, we should
impose the same constraint that prices are non-discriminatory  the same price p
is offered to each agent.  So lets assume that our mechanism is fixed to
choosing a single price, then offering this price to each buyer (in sequence).

Note: For any fixed p, and for any ordering of the players (even if we can
approach each player multiple times) there is a unique equilibrium outcome: a
player will consider purchasing only if it is the last time he or any of his
neighbors will be approached, in which case he will purchase iff his value is
greater than p.
è Conclusion: never worthwhile to approach a player multiple times.


This implies that it is always optimal to set p equal to the Myerson reserve
price.   Also, the revenue is equal to Myerson revenue * size of maximal
independent set that occurs when nodes are added greedily, in the reverse of the
order in which the mechanism approaches them.
So if the mechanism can choose the ordering, it can obtain Myerson revenue *
size of maximum independent set, and this is best possible.


The main difference between simultaneous and sequential mechanisms is that the
outcome for the sequential mechanism is always integral (each agent either
buys iff value > price, or never buys), whereas solutions for the simultaneous
mechanism can be fractional (agents can choose purchase thresholds that arent
either p or 1).  In particular, any outcome of a sequential mechanism is also an
equilibrium in the simultaneous mechanism.

Question: how does worst-case revenue compare?  (i.e. worst-case equilibrium vs.
worst-case ordering)
Answer: unbounded.  We have a 5-cycle example showing that worst-case
fractional solution can be much worse than the worst-case integral solution.
 So we can have [worst-case in sequential] >>>>> [worst-case in simultaneous].

Question: how does best-case revenue compare?  (i.e. best-case equilibrium vs.
best-case ordering)
Answer: they are equal.  To see this, note that a fractional solution to the min
dominating set problem, subject to the constraint that
   $[x_i > 0] \Rightarrow [x_i + sum_{j \in N_i} x_j = 1]$,
can be converted into an integral solution without loss  think of repeatedly
choosing some $i$ such that $x_i > 0$ and combining $x_i$ and all of the
$x_j$s for neighbours of $i$ into node $i$.  After doing this repeatedly, we
end up with a solution that is no better than an integral solution, and each
step is without loss.

Slightly unrelated result:
In the clique, if the mechanism can commit to an arbitrary price vector, then
revenue converges to 1/e as n grows large.
Compare with 0.288 with no price commitment.

\mfcomment{The following is taken from an email by David, May 23, 2012.}
Brendan and I did some calculations earlier today for the n-clique with subgame
perfect prices.
Unless we made some mistakes (a distinct possibility), we get that
the first person in an n-clique is offered a price of
$P(n) := \prod_{k=1}^n (1-2^{-k})$.
In particular, this is monotone increasing in $n$.
The seller's total expected revenue is
$(1-2^{-n}) \cdot P(n)$.

As n goes to infinity, both converge to some number, which is roughly 0.2888.
Not too much larger than 0.25, but then again, it's not clear how much larger we
should expect.


